Accelerating CNN inference on FPGAs: A Survey

Convolutional Neural Networks (CNNs) are currently adopted to solve an ever greater number of problems, ranging from speech recognition to image classification and segmentation. The large amount of processing required by CNNs calls for dedicated and tailored hardware support methods. Moreover, CNN workloads have a streaming nature, well suited to reconfigurable hardware architectures such as FPGAs. The amount and diversity of research on the subject of CNN FPGA acceleration within the last 3 years demonstrates the tremendous industrial and academic interest. This paper presents a state-of-the-art of CNN inference accelerators over FPGAs. The computational workloads, their parallelism and the involved memory accesses are analyzed. At the level of neurons, optimizations of the convolutional and fully connected layers are explained and the performances of the different methods compared. At the network level, approximate computing and datapath optimization methods are covered and state-of-the-art approaches compared. The methods and tools investigated in this survey represent the recent trends in FPGA CNN inference accelerators and will fuel the future advances on efficient hardware deep learning.

==> table/Para.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
Parallelism   & Inter-FM & \multicolumn{2}{c|}{Intra-FM} & Inter-Ker & \multicolumn{2}{c|}{Intra-Ker} \\ \hline
Loop 		  & $L_N$    & $L_V$         & $L_U$         & $L_C$     & $L_J$              & $L_K$        \\ \hline
Unroll factor & $P_N$    & $P_V$         & $P_U$         & $P_C$     & $P_J$              & $P_K$        \\ \hline
Tiling Factor & $T_N$    & $T_U$         & $T_U$         & $T_C$     & $T_J$              & $T_K$        \\ \hline
\end{tabular}

==> table/PopularDatasets.tex <==
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Dataset                           & Sample Resolution & \#Classes & \#Train/Val Samples & \#Test Samples & Application                                                                                        \\ \hline
MNIST \cite{Lecun1990}          & 28 x 28 x 3       & 10        & 60 K                            & 10 K           & Digit classification                                                                   \\ \hline
Cifar10 \cite{Krizhevsky2009}   & 32 x 32 x 3       & 10        & 50 K                            & 10 K           & \multirow{3}{*}{Image Classification}                                                              \\ \cline{1-5}
Cifar100 \cite{Krizhevsky2009}  & 32 x 32 x 3       & 100       & 50 K                            & 10 K           &                                                                                                    \\ \cline{1-5}
ImageNet \cite{Deng2009}        & 256 x 256 x 3     & 1000      & 1.3 M                           & 100 K          &                                                                                                    \\ \hline
PascalVOC \cite{Everingham2015} & -                 & 20        & 11.5 K                          & -              & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Classification , Detection\\ Segmentation\end{tabular}} \\ \cline{1-5}
COCO \cite{Lin2014}      & -                 & 91        & 328 k                           & -              &                                                                                                    \\ \cline{1-5}
Openimages \cite{Krasin2016}    & -                 & 5000      & 9 M                             & 125.4 K        &                                                                                                    \\ \hline
\end{tabular}


==> tikz/conv.tex <==
% \documentclass[tikz]{standalone}
% \usepackage{tikz-dimline}
% \pgfplotsset{compat=newest}
% \begin{document}
\begin{tikzpicture}[scale=0.4,every node/.style={scale=0.7}]]
	% In Feature maps
	\draw [fill=white](0,0,0) rectangle (4,4,0);
	\draw [fill=red!20!white]	(0,3,0) rectangle (1,4,0);
	\draw [fill=white](0,0,2) rectangle (4,4,2);
	\draw [fill=red!20!white]	(0,3,2) rectangle (1,4,2);
	\draw [fill=white](0,0,4) rectangle (4,4,4);
	\draw [fill=red!20!white]	(0,3,4) rectangle (1,4,4);

	% Filters
	\draw [fill=cyan!40!white]	(7,0,-12) rectangle (8,1,-12);
	\draw [fill=cyan!40!white]	(7,0,-11) rectangle (8,1,-11);
	\draw [fill=cyan!40!white]	(7,0,-10) rectangle (8,1,-10);

	\draw [fill=yellow!85!white]	(7,0,-7) rectangle (8,1,-7);
	\draw [fill=yellow!85!white]	(7,0,-6) rectangle (8,1,-6);
	\draw [fill=yellow!85!white]	(7,0,-5) rectangle (8,1,-5);

	\draw [fill=green!40!white]	(7,0,-2) rectangle (8,1,-2);
	\draw [fill=green!40!white]	(7,0,-1) rectangle (8,1,-1);
	\draw [fill=green!40!white]	(7,0,0) rectangle  (8,1,0);

	\draw [fill=blue!40!white]	(7,0,3) rectangle (8,1,3);
	\draw [fill=blue!40!white]	(7,0,4) rectangle (8,1,4);
	\draw [fill=blue!40!white]	(7,0,5) rectangle (8,1,5);

	\draw [fill=red!40!white]	(7,0,8)  rectangle (8,1,8);
	\draw [fill=red!40!white]	(7,0,9)  rectangle (8,1,9);
	\draw [fill=red!40!white]	(7,0,10) rectangle (8,1,10);

	% Out Feature maps
	\draw [fill=cyan!40!white]	(15,0,-2) 	rectangle (18,3,-2);
	\draw [fill=yellow!85!white](15,0,0) 	rectangle (18,3,0);
	\draw [fill=green!40!white]	(15,0,2) 	rectangle (18,3,2);
	\draw [fill=blue!40!white]	(15,0,4) 	rectangle (18,3,4);
	\draw [fill=red!40!white]	(15,0,6) 	rectangle (18,3,6);

	% Sizes
		% Kernels
		\node at (9,0.5,-12)	{$K$}; %Was R
		\node at (7.5,2,-12)	{$K$};
		\node at (6,1.5,-11)	{$C$};
		\node [rotate=45] at (9.3,-0.3,-6) 		{$N \times C$};
		\path [<->] (7,1.5,-12)  edge (8,1.5,-12);
		\path [<->] (8.2,0,-12) edge (8.2,1,-12);
		\path [<->] (6.8,1.2,-10) edge (6.8,1.2,-12);
		\path [<->] (8.3,-0.3,10) edge (8.3,-0.3,-12);
		% In FMs
		\node at (-1.3,2,4)		{$H$};
		\node at (2,5,0)		{$W$};
		\node at (-0.8,4.5,2)	{$C$};
		\path [<->] (0,4.5,0)  edge (4,4.5,0);
		\path [<->] (-0.5,0,4) edge (-0.5,4,4);
		\path [<->] (-0.2,4.2,0) edge (-0.2,4.2,4);
		% Out FMs
		\node at (16.5,4,-2)	{$U^{}$};
		\node at (19.5,1.5,-2)	{$V^{}$};
		\node at (19,-1,2)		{$N^{}$};
		\path [<->] (15,3.5,-2)  edge (18,3.5,-2);
		\path [<->] (18.5,0,-2) edge (18.5,3,-2);
		\path [<->] (18.2,-0.3,6) edge (18.2,-0.3,-2);

	% Focus on the red one
	\draw [fill=red] 		(15,2.5,6) 	rectangle (15.5,3,6);
	\path [style=dashed] 	(15,2.75,6) edge (8,0,10);
	\path [style=dashed] 	(15,2.75,6) edge (8,0,8);
	\path [style=dashed] 	(7,1,10) 	edge (0,4,4);
	\path [style=dashed] 	(7,1,8)		edge (0,4,0);

	% Titles
	\node at (-2,-3,0) {Input feature maps $\matr{X}$};
	\node at (8,-1,10) {Convolution Filters $\Theta^{}$};
	\node at (15,-3,3) {Output feature maps $\matr{Y}$};

\end{tikzpicture}

% \end{document}

% \dimline    [color=blue,
% 			line style={thick},
% 			extension start style={blue,thin},
% 			extension end style={blue,thin}
% 			]{($(E)+(0,.5)$)}{($(G)+(0,.5)$)}{$t_c$};


==> tikz/mlp.tex <==
\def\layersep{2.5cm}

\begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep]
    \tikzstyle{every pin edge}=[<-,shorten <=1pt]
    \tikzstyle{neuron}=[circle,fill=black!25,minimum size=17pt,inner sep=0pt]
    \tikzstyle{input neuron}=[neuron, fill=green!50];
    \tikzstyle{output neuron}=[neuron, fill=red!50];
    \tikzstyle{hidden neuron}=[neuron, fill=blue!50];
    \tikzstyle{annot} = [text width=4em, text centered]

    % Draw the input layer nodes
    \foreach \name / \y in {1,...,4}
    % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
        \node[input neuron, pin=left:Input \#\y] (I-\name) at (0,-\y) {};

    % Draw the hidden layer nodes
    \foreach \name / \y in {1,...,5}
        \path[yshift=0.5cm]
            node[hidden neuron] (H-\name) at (\layersep,-\y cm) {};

    % Draw the output layer node
    \node[output neuron,pin={[pin edge={->}]right:Output}, right of=H-3] (O) {};

    % Connect every node in the input layer with every node in the
    % hidden layer.
    \foreach \source in {1,...,4}
        \foreach \dest in {1,...,5}
            \path (I-\source) edge (H-\dest);

    % Connect every node in the hidden layer with the output layer
    \foreach \source in {1,...,5}
        \path (H-\source) edge (O);

    % Annotate the layers
    \node[annot,above of=H-1, node distance=1cm] (hl) {Hidden layer};
    \node[annot,left of=hl] {Input layer};
    \node[annot,right of=hl] {Output layer};
\end{tikzpicture}
% End of code
\end{document}

